PlaceRaider: Virtual Theft in Physical Spaces with Smartphones

As smartphones become more pervasive, they are increasingly targeted by malware. At the same time, each new generation of smartphone features increasingly powerful onboard sensor suites. A new strain of sensor malware has been developing that leverages these sensors to steal information from the physical environment (e.g., researchers have recently demonstrated how malware can listen for spoken credit card numbers through the microphone, or feel keystroke vibrations using the accelerometer). Yet the possibilities of what malware can see through a camera have been understudied. This paper introduces a novel visual malware called PlaceRaider, which allows remote attackers to engage in remote reconnaissance and what we call virtual theft. Through completely opportunistic use of the camera on the phone and other sensors, PlaceRaider constructs rich, three dimensional models of indoor environments. Remote burglars can thus download the physical space, study the environment carefully, and steal virtual objects from the environment (such as financial documents, information on computer monitors, and personally identifiable information). Through two human subject studies we demonstrate the effectiveness of using mobile devices as powerful surveillance and virtual theft platforms, and we suggest several possible defenses against visual malware.

==> ack.tex <==
% !TEX root = main.tex

\section*{Acknowledgment}

This material is based upon work supported by the National Science Foundation under Grant No. 1016603. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the author(s) and do not necessarily reflect the views of the National Science Foundation. We thank John McCurley for his editorial help.

==> conclusion.tex <==
% !TEX root = main.tex

\section{Conclusion}
\label{sec:conclusion}
In this paper we introduce a new general threat to the privacy and physical security of smartphone users that we call virtual theft. We conceptualize a mode of attack where opportunistically collected data is used to build 3D models of users' physical environments. We demonstrate that large amounts of raw data can be collected and define novel approaches that can be used to improve the quality of data that is sent to the attacker. We offer \sys, an implementation of a virtual theft attack and through 
human subject studies demonstrate that such attacks are feasible and powerful. An ancillary contribution is our work addressing the use of existing \sfm tools in indoor spaces with poor quality images.

==> discussion.tex <==
% !TEX root = main.tex

\section{Discussion}
\label{sec:disc}

We first discuss how \sys can be improved from an attack perspective
and then we discuss various possible defenses against such visual
malware.

\subsection{Improvements to the attack}

\xhdr{Targeted \sys.}  While providing a very general and powerful
surveillance capability, our implementation of \sys relies solely on
human vision for the extraction of detailed valuable information. A
desired capability might include autonomous (machine) identification
and extraction of sensitive data. Existing computer vision methods in
object recognition and image matching~\cite{sift} could be
employed to look for a pre-defined set of objects of interest, as could
optical character recognition or bar code
recognition  to glean text and
other sensitive data from the scene. In doing this an interesting question is
whether the 3D context provided by our reconstructions could improve
object recognition over baseline algorithms that simply scan through
the raw images.

\xhdr{Improving \vtsw data reduction.}
While we were able to demonstrate successful data reduction averaging
more than 73\%, many of the images in the reduced sets still had poor
quality and high redundancy.  There are at least two possible potential methods to
improve data reduction using orientation and acceleration data. The
first involves utilizing the acceleration data that is already logged,
but not utilized, by the \sys app. If proper signal processing were
applied to the acceleration data, it might be possible to infer
instantaneous movement at the time of image capture. Such a capability
would allow velocity thresholds to be applied to images, 
ignoring images likely to have significant motion blur.
 A second method to improve data
reduction would be removal of redundant images at the global
level. Our current implementation removes redundant
images by looking only at local temporal neighbors. An alternative
approach would be to use the camera gyroscopes to record where the
camera has pointed before, and to take photos only when it is oriented towards new, unseen directions.
Such approaches will become more feasible as smartphones incorporate increasingly accurate
sensors.

While the anisotropic quality metric was effective at reducing the
size of our image sets, manual inspection of the subsets revealed
regular occurrences of grossly under- or over-exposed images. An
improvement of our reduction technique could target luminance
distributions of images, thus targeting and discarding additional poor
quality images. We leave exploration of this and the other suggested
data reduction improvements for future work.

\xhdr{Improving the 3D models.}  In the past, large-scale
structure-from-motion algorithms  typically have been used for outdoor
scenes using images purposefully taken by photographers. In
Section~\ref{sec:eval} we showed that Bundler and PMVS successfully
generated models on our opportunistically collected images of indoor
spaces. This new domain raises interesting computer vision questions
about how to improve 3D model generation with more difficult image
collections.  One possible direction is to explore alternative
algorithms for feature identification and comparison that would work
better in indoor spaces (where illumination is more variable and
distinct features are less common because of the many plain  surfaces).
It would also be interesting to use recent work that uses stronger
assumptions about a scene, for example that the scene has many flat planes,
to produce more accurate models for indoor scenes~\cite{5459145}.  We
leave this exploration for future work.

Another interesting direction is to understand why
the datasets from some of our 20 test subjects produced  much better
models than others. In some cases this can explained simply by  the size
of the datasets, but in other cases there are clearly other unknown factors
at work. These may relate to the lighting conditions in the room at different
times of the day, or to the smartphone usage habits of different people (e.g. the 
amount they move while using the phone, or how often their fingers accidentally
cover the smartphone lens).

\subsection{Defenses}

We have shown that virtual theft is a compelling threat to privacy. Visual malware is a nascent area that requires more research. While existing work has established visual attacks~--- we discuss some in Section~\ref{sec:related}~--- \sys introduces a threat that requires a different defense. While evaluation of defenses is outside of the scope of this paper, we offer these possible solutions for seeding future work.

\xhdr{Permissions and defense.}
We detailed the  set of Android permissions needed by \sys in Section~\ref{sec:overview}. Previous work has shown that permission sets can be partitioned by splitting malware functionality and permissions among multiple applications and using covert channels to communicate~\cite{soundcomber}. Such covert channels are limited in channel capacity and preclude their use for transmitting image or other sensor data between applications. This limitation allows us to safely assume that \sys can only be employed when the user accepts the application permissions at installation. 
Static permission checking can be performed automatically, but again, since common camera apps require similar permissions, we do not expect such mechanisms to provide a successful defense~\cite{Nauman:2010:AEA:1755688.1755732,Enck08mitigatingandroid}.

This points to the obvious recommendation that users should be cautious about what they install, and download apps only from trusted software developers.  In general, users should be suspicious of apps that have access to the camera and the Internet. 

\xhdr{Persistent shutter sound.}  We described in
Section~\ref{sec:collection} the measures that Android devices take to
`require' a shutter sound when taking photographs and our trivial, but
effective, method to circumvent this by muting the speaker. An inability to prevent the
shutter sound would foil \sys's attempts to control the camera without
detection.  A persistent shutter sound, possibly with dedicated
hardware that is impervious to overrides by software, is a recommended
approach that would provide a complete defense against \sys. This
obviously requires initiatives by hardware manufacturers.

\xhdr{Permissions for sensors.}
Current Android and iOS operating systems require no permissions to access acceleration or gyroscope data despite the high rates of collection and accuracy that they possess.	 An explicit permission to use the sensor resources would not prevent virtual theft, as \sys only uses this data to further reduce the image set, but would increase the security of mobile devices; existing work has demonstrated attacks using accelerometers to analyze keystrokes, for example~\cite{spiphone,Miluzzo:2012:TYF:2307636.2307666,Owusu:2012:API:2162081.2162095}. While we offer this as a defense, it would only minimally~--- if at all~--- preserve privacy, as there would be no prevention of the collection and transmission of images.

\xhdr{Hardware protections.} One possibility is to enhance the operating system architecture to allow photographs and video to be captured only when a physical button is pressed. Such a mechanism may prevent surreptitious capture of photographic data, but may prevent novel uses of the camera by legitimate applications.

\xhdr{\sys detector.}
There is no logical motivation for users to intentionally take poor-quality photos that have any combination of improper focus, motion blur, improper exposure, or unusual orientations/twist. Just as \sys can use methods to parse images to maximize quality, the Android operating system can potentially assess each photo at time of capture, or over longer periods of time, and ask the user to confirm that they desire these images. Such an approach might frustrate \sys attempts to perform long-running image collection. 

\sys differs from most legitimate camera applications in that individual photos are taken without input from the user interface. The API could possibly be modified such that certain security-related methods would require invocation linked to user input. This would allow a total defense against \sys, as attempts to take photos in a stealthy manner would be thwarted. We leave exploration of these approaches, including attempts to estimate their efficacy as a defense, for future research.

\xhdr{Physical camera discipline.}
Successful virtual theft requires that the mobile phone, in physical control of the user, be in a position to take photographs. Organizational policies against possession of camera-containing devices~--- such policies are commonly in place in sensitive areas~--- and personal discipline can both serve to prevent disclosure of sensitive images despite the capability of malicious apps.






==> related.tex <==
% !TEX root = main.tex
\section{Related Work}
\label{sec:related}

\xhdr{Sensory malware.}  The prevalence of malware on mobile platforms
is the focus of considerable research. Recent work shows more than
1,200 active variants of malware in the Android ecosystem that are
largely impervious to attempts to prevent their
exploitation~\cite{zhou2012}. An emerging threat is that of sensory
malware, which works by leveraging the varied sensors of mobile
devices. Demonstrations include using microphones to obtain dialed or
spoken account information~\cite{soundcomber} and keyloggers that
operate via structure-borne vibrations measured through an
accelerometer~\cite{spiphone,Miluzzo:2012:TYF:2307636.2307666,Owusu:2012:API:2162081.2162095}. Despite
recent attention given to sensory malware, there is a notable absence
of examples that recruit the camera. One example is the Stealthy Video
Capturer~\cite{Xu:2009:SVC:1514274.1514285}. This approach, while now
dated and not reflective of the current generation of mobile devices,
does present a clever method to collect image data in a stealthy
manner. This type of system applied to modern Android devices would
bear resemblance to the data collection segment of \sys. Where \sys
differs is that we seek sampling of image data at a lower rate (0.5
frame per second vs. video frame rates) and for longer periods of
time. Further, our efforts to reduce data and generate unified
structures (3D models) to describe personal spaces further
differentiate \sys as previous work did not attempt to make sense of
the data that is collected.

\xhdr{Imaging privacy attacks.}
Imaging attacks are unique in that they require a line of sight~--- direct or indirect via diffraction, reflection, and refraction~--- between the attacker and the target source (victim). In standard parlance, ``standoff'' refers to the physical distance between the attacker and target source.
The preponderance of documented imaging attacks offer varying standoff distances, but are asymptotically limited to physical visual limitations.
These examples of visual attacks on privacy require dedicated, and often advanced, imaging devices. One category of these attacks seeks to spy on active electronic displays. This can be accomplished with photomultipliers~\cite{1004358} or long focal length optics that can even extract information from reflections of the source image~\cite{5207653,4531151}.
Keylogging via imaging can be accomplished using techniques similar to the aforementioned attacks~\cite{DBLP:conf/ccs/RaguramWGMF11} or with thermal cameras~\cite{Mowery:2011:HMC:2028052.2028058}. A particularly unique visual attack can physically copy keys using images of target keys~\cite{Laxton:2008:RPK:1455770.1455830}. While all of these attacks are compelling, they require  use of methods where attackers (or their specialized hardware) are in optical range (the physical vicinity) of the victim. \sys has a unique property in that it allows standoff distances limited only by the reach of the Internet, yet remains intimately close to the victim by leveraging the victim's own camera and sensors.
 
\xhdr{Defenses.}
Several security enhancements have been proposed for Android. We encourage the reader to review Bugiel et al.'s report~\cite{TUD-CS-2011-0127} for a thorough review of these approaches.  In general, these approaches can check permissions at installation time~\cite{Nauman:2010:AEA:1755688.1755732,Enck08mitigatingandroid}, monitor runtime permission usage~\cite{Ongtang:2009:SRA:1723192.1723245},
regulate inter-application communication to defeat confused deputy attacks~\cite{Enck08mitigatingandroid,DBLP:journals/corr/abs-1102-2445,Felt:2011:PRA:2028067.2028089,xmandroid-ndss},  
mitigate covert channels~\cite{TUD-CS-2011-0127}, 
and track the flow of sensitive data~\cite{Enck:2010:TIT:1924943.1924971,Portokalidis:2010:PAV:1920261.1920313}. 

As detailed in Section~\ref{sec:overview}, \sys can be deployed in a legitimate-looking camera application as a Trojan, as they share like permissions, and does not rely on covert communication. As such, there is no need for escalating privileges, so the bulk of existing defenses aimed at enforcing granted permissions offer little protection against \sys. 
However, context sensitive permission checks during runtime might be an effective defense against Trojans attempting to steal private data. Porscha~\cite{Conti:2010:CCP:1949317.1949355} can provide such granular control for content that originates external to the phone, but does not provide protection provisions for data generated by the phone as would be necessary for \sys. Systems like CRePE~\cite{Ongtang:2010:PPO:1920261.1920295} can provide greater levels of protection but cannot work without modifications to existing Android middle-ware.


Cai's framework for defending against sensory malware attacks offers several promising methods to thwart malicious apps~\cite{Cai:2009:DAS:1592606.1592614}. 

Because \sys's behavior is comparable to legitimate camera apps and only requires communication to the \sys command and control server, this defensive approach would be inadequate. 

The sole behavioral differences between \sys and legitimate camera applications from the system's perspective are the rate of data collection and frequent transmission of images to an off-board server. This might make \sys subject to detection via Cai's proposed information flow tracking, but ceasing the function of \sys on the basis of its behavior would also work to keep many legitimate camera apps from operating.

VirusMeter~\cite{Liu:2009:VPY:1691138.1691155} is an application that seeks to identify malicious applications through their anomalous power profiles. This approach would only be effective against \sys if the rate of activity was high enough to result in an anomalous power profile.



